Metrics Dashboard: A Hosted Platform for Software Quality Metrics

There is an emerging consensus in the scientific software community that progress in scientific research is dependent on the "quality and accessibility of software at all levels" (wssspe.researchcomputing.org.uk/). This progress depends on embracing the best traditional---and emergent---practices in software engineering, especially agile practices that intersect with the more formal tradition of software engineering. As a first step in our larger exploratory project to study in-process quality metrics for software development projects in Computational Science and Engineering (CSE), we have developed the Metrics Dashboard, a platform for producing and observing metrics by mining open-source software repositories on GitHub. Unlike GitHub and similar systems that provide individual performance metrics (e.g. commits), the Metrics Dashboard focuses on metrics indicative of team progress and project health. The Metrics Dashboard allows the user to submit the URL of a hosted repository for batch analysis, whose results are then cached. Upon completion, the user can interactively study various metrics over time (at varying granularity), numerically and visually. The initial version of the system is up and running as a public cloud service (SaaS) and supports project size (KLOC), defect density, defect spoilage, and productivity. While our system is by no means the first to support software metrics, we believe it may be one of the first community-focused extensible resources that can be used by any hosted project.

==> details.tex <==
% STUFF KL deleted from II Related Work


The same authors~\cite{shah_software_2013} later compared two different variants of defect density: \emph{standard} (steadily increasing variability) and \emph{differential} (large variability) and concluded that the standard defect density provides a global quality view of the project (with all history included), while differential defect density provides a local quality view (specific to a version of the project).


Nagappan and Ball~\cite{nagappan_static_2005} looked into the effectiveness of static analysis tools in predicting pre-release defect density and found that these tools were not as effective at detecting deep logical or design errors as human developers.



%%% ARCHITECTURE

In the design and implementation of the \systemname{}, we have relied on methods and insights from \emph{software architecture}, ranging from the seminal report by Garlan and Shaw~\cite{garlan_introduction_1994} to the updated reference by Bass et al.~\cite{bass_software_2012}. 
In particular, \emph{(enterprise) application integration} techniques~\cite{hohpe_enterprise_2003} and RESTful web services~\cite{richardson_restful_2007,webber_rest_2010} form the architectural basis for the \systemname.


%earlier work on test effectiveness - not cited in this paper
%IEEE Transactions on Reliability
%\cite{lyu_coverage_1994}




% STUFF GKT deleted from IV.
% Too low-level for an academic paper.
\begin{itemize}
\item authenticated login via GitHub (optional). This is how any open source developer on GitHub can log into request that we add projects to the dashboard. It is optional, because the primary purpose of the dashbord 
\item latest visualizations - briefly outlined in section 4.3.
\item explore current projects
\item for each project, we see
	\begin{itemize}
    \item latest project data: metric = density and frequency = week, e.g.
    	\begin{itemize}
        \item \url{https://tirtha.loyolachicagocs.org/metrics/api/spoilage/astropy/astropy/master?groupBy=week}
        \end{itemize}
    \item latest project data: metric = spoilage and frequency = month, e.g.
    	\begin{itemize}
        \item \url{https://tirtha.loyolachicagocs.org/metrics/api/spoilage/astropy/astropy/master?groupBy=month}
        \end{itemize}
    \item GitHub API data for a chosen project or authenticated private user
    \item project information and further details
	    \begin{itemize}
    	\item \url{https://luc-metrics.herokuapp.com/projects/56c122dcd8a8acec237e7a06}
    	\end{itemize}
    \item weekly dashboard for a chosen project, e.g.
    	\begin{itemize}
        \item	\url{https://luc-metrics.herokuapp.com/dash/public/week/astropy}
        \end{itemize}
    \item monthly dashboard for a chosen project. e.g.
    	\begin{itemize}
        \item \url{https://luc-metrics.herokuapp.com/dash/public/month/astropy}
        \end{itemize}
    \item health summary for a chosen project, e.g.
    	\begin{itemize}
        \item \url{https://luc-metrics.herokuapp.com/health/astropy}
        \end{itemize}
    \item stats summary for a chosen project, e.g.
    	\begin{itemize}
        \item \url{https://luc-metrics.herokuapp.com/stats/astropy}
        \end{itemize}
    \end{itemize}
\item can also add a project to track
	\begin{itemize}
    \item request form is available at the following URL,
    	\begin{itemize}
        \item \url{https://luc-metrics.herokuapp.com/other/requests/track}
        \end{itemize}
	\item form gets submitted for batch processing 
    \item request information shows up under pending, e.g.
    	\begin{itemize}
        \item \url{https://luc-metrics.herokuapp.com/projects/pending}
        \end{itemize}
    \item until it becomes available under current, e.g.
    	\begin{itemize}
        \item \url{https://luc-metrics.herokuapp.com/projects}
        \end{itemize}
	\end{itemize}
\end{itemize}

\subsection{\systemname{}\ RESTful API}
\todo[inline]{laufer: opening par}

\begin{itemize}
\item sample GET routes include
	\begin{itemize} 
    \item \texttt{/dash/public/\{frequency\}/\{project\}}
	\item \texttt{/dash/public/\{period\}/\{metric\}/\{project\}}
    \end{itemize}
\item sample POST routes include
	\begin{itemize}
	\item \texttt{/other/requests/track}
    \end{itemize}
\end{itemize}    
    
where    

\begin{itemize}    
\item frequency = week | month
\item metric = density | kloc | spoilage
\item additional = issues for a chosen project, e.g.
	\begin{itemize}
    \item open | closed | openCumulative | closedCumulative
    \end{itemize}
\end{itemize}

These RESTful API resources are metric-centric in the sense that one first chooses the metric with its attributes, then the project. In the future, it is conceivable that the \systemname{} will support project- and team-centric resources such as
\begin{itemize}
\item \texttt{/dash/public/\{project\}/\{metric\}}
\item \texttt{/dash/public/\{team\}/\{metric\}}
\end{itemize}

\subsection{\systemname{} web application}

The client-side application is currently available for initial testing at the following URL,

\begin{itemize}
\item \url{https://luc-metrics.herokuapp.com/}
\end{itemize}

This web application has primarily been designed and developed as a public reference and visualization interface for the current exposed metrics' services, as detailed above. The default view is public, thereby enabling a non-authenticated user to sample current tracked software projects, as curated by the \systemname{} project.

\subsection{Tracked projects and requests}

A public, non-authenticated user may select a tracked project, and quickly assess project metrics using the provided dashboard visualizations. A detailed record of each tracked project is maintained in our MongoDB database, which is publicly exposed using an Express and Node.js API. A sample URL for this API is as follows,

\begin{itemize}
\item \url{https://luc-metrics.herokuapp.com/api/projects/}
\end{itemize}

A user may also request additional projects for tracking, which are then assessed as part of the pending project. Successful project assessment and review permits a transition to an actively tracked project, thereby enabling visualization of project metrics through the application's dashboard.

